On the Interplay Between Sparsity and Training in Deep Reinforcement Learning

We study the benefits of different sparse architectures for deep reinforcement learning. In particular, we focus on image-based domains where spatially-biased and fully-connected architectures are common. Using these and several other architectures of equal capacity, we show that sparse structure has a significant effect on learning performance. We also observe that choosing the best sparse architecture for a given domain depends on whether the hidden layer weights are fixed or learned.

==> sections/overview.tex <==

Points to make:
\begin{enumerate}
    \item Sparse structure plays a key role in a deep RL system's ability to generalize its knowledge.
    \item The extent to which sparse structure helps a system generalize depends on the environment.
    \subitem Our study provides deeper insight into when this holds for Minitar. 
    \subitem Maybe an observation worth making: Does this depend on other factors too?
\end{enumerate}


Claims:
\begin{enumerate}
    \item (Minor) The extent to which sparse structure helps a deep RL system generalize depends on the environment.
    \item (Major) The extent to which backprop improves generalization depends on the sparse structure and on the environment.
    \begin{enumerate}
        \item This has consequences to sparse structures that derive from end-to-end learning (e.g. L1). 
        \item There is supporting evidence for this in the literature (See \citet{rahimi_recht_kernels, rahimi_recht_weighted_sums_RKS_08}). However, they don't make the connection that our experiments make; for instance, they demonstrate how random fixed networks can perform on par with learned networks in the supervised setting. Though, we are---to our knowledge---the first to observe this in RL. And Rahimi and Recht never emphasized the environment's role in this phenomenon (i.e., the data distribution's role).
        \item Some sparse structures are useful only when we learn the weight magnitudes. 
    \end{enumerate}
    \item (Minor) Surprisingly, spatial structure---which convolutional architectures exploit---is not always the most performant in domains with spatial dynamics.
    \item (Minor) Provided further evaluation of predictive sparsity.
\end{enumerate}
